Relphormer: Relational Graph Transformer for Knowledge Graph Representations

Transformers have achieved remarkable performance in widespread fields, including natural language processing, computer vision and graph mining. However, vanilla Transformer architectures have not yielded promising improvements in the Knowledge Graph (KG) representations, where the translational distance paradigm dominates this area. Note that vanilla Transformer architectures struggle to capture the intrinsically heterogeneous structural and semantic information of knowledge graphs. To this end, we propose a new variant of Transformer for knowledge graph representations dubbed Relphormer. Specifically, we introduce Triple2Seq which can dynamically sample contextualized sub-graph sequences as the input to alleviate the heterogeneity issue. We propose a novel structure-enhanced self-attention mechanism to encode the relational information and keep the semantic information within entities and relations. Moreover, we utilize masked knowledge modeling for general knowledge graph representation learning, which can be applied to various KG-based tasks including knowledge graph completion, question answering, and recommendation. Experimental results on six datasets show that Relphormer can obtain better performance compared with baselines. Code is available in https://github.com/zjunlp/Relphormer.

==> tables/DatasetStatictics-KGQA.tex <==
\begin{table}[]
% \begin{spacing}{1.1}
\renewcommand\arraystretch{1.2}

\caption{Statistics for FreebaseQA and WebQuestionSP datasets}


\begin{tabular}{lccccc}

\toprule


\multirow{2}{*}{Dataset} & \multicolumn{2}{l}{\textbf{FreebaseQA}} & \multicolumn{2}{l}{\textbf{WebQuestionSP}} \\ \cline{2-5} 
 & Full & Filtered & Full & Filter \\
 
\midrule

Train & 20,358 & 3,713 & 3,098 & 850 \\
Test & 3,996 & 755 & 1,639 & 484  \\   

\bottomrule

\end{tabular}

\label{tab:Dataset_Statistics_KGQA}

\end{table}

==> tables/DatasetStatistics-Codex.tex <==
\begin{table}[!t]
    \caption{Imbalanced Knowledge Graph Completion Statistics.}
        \label{table:1}
    \centering
    % \setlength{\belowcaptionskip}{-0.5cm}
    \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{cccc}
            \toprule
            \textbf{Dataset}  & \textbf{\#Relations} & \textbf{\#Entities} & \textbf{\#Train Triples}  \\
            \midrule
            % Codex-large & 69 & 77,951 & 551,193 \\
            Codex-large-\textbf{imb} & 54 & 4,380 & 12,420 \\
            \bottomrule
        \end{tabular}
    }
\end{table}

==> tables/DatasetStatistics-KG-ReC.tex <==
\begin{table}[!t]
        \caption{Statistics for Knowledge Graph Recommendation }
        \centering
        % \setlength{\belowcaptionskip}{-0.5cm}
        \resizebox{0.4\textwidth}{!}{
            \begin{tabular}{cccccc}
                \toprule
                \textbf{Dataset}  & \textbf{\#users} & \textbf{\#items} & \textbf{\#actions} & \textbf{\#Avg. length} & \textbf{\#Density}\\
                \midrule
                ML-20m & 138,493 & 26,744 & 20m & 144.4 & 0.54\%\\   
                \bottomrule
            \end{tabular}
        }
    \label{tab:Dataset_Statistics_KG_Rec}
\end{table}

==> tables/DatasetStatistics-KGC.tex <==
\begin{table}[!t]
        \caption{Statistics of KG completion datasets.}
        \centering
        % \setlength{\belowcaptionskip}{-0.5cm}
        \resizebox{0.4\textwidth}{!}{
            \begin{tabular}{cccccc}
                \toprule
                \textbf{Dataset}  & \textbf{\#Rel.} & \textbf{\#Ent.} & \textbf{\#Train}  & \textbf{\#Dev} & \textbf{\#Test}\\
                \midrule
                FB15K-237 & 237 & 14,541 & 272,115 & 17,535 & 20,466
                \\    
                WN18RR & 18 & 40,943 & 141,442 & 5,000 & 5,000
                \\    
                UMLS & 46 & 135 & 5,216 & 652 & 661 
                \\
                \bottomrule
            \end{tabular}
        }
        \label{tab:Dataset_Statistics_KGC}
\end{table}

==> tables/Inference_Time.tex <==
\begin{table}[!t]

    \caption{
    Comparisons with KG-BERT and StAR on FB15K-237. 
    % $\dagger$mean initialization with \texttt{BERT-base}.
    “T/Ep” stands for time per training epoch and “Infer” denotes inference time on test set. The time was collected on one 1080-Ti GPU.
    } 

    \centering
        \scalebox{0.85}{
    \begin{tabular}{lllll|ll}
    \toprule
    & \textbf{Hits@1} &  \textbf{@3}  & \textbf{@10}  & \textbf{MRR} & \textbf{T/Ep} & \textbf{Infer}\\ 
    \midrule
    
    KG-BERT & - & - & .420  & - & $\approx$10h &  $\approx$1500h \\
    % StAR-roberta & .205* & .322* & .482*  & .296* & $\approx$9.5h & $\approx$8h  \\
    StAR & .162 & .255 & .400  & .240 & $\approx$9.5h & $\approx$8h  \\
    \textbf{Relphormer} &  \textbf{.314} & \textbf{.393} & \textbf{.481}   &  \textbf{.371} & $\approx$1.5h & $ \approx 5m$ \\
    
    
    \bottomrule

    \end{tabular}
    }
   
 \label{tab:inference_time}


\end{table}

==> tables/KGQA.tex <==
\begin{table}[]
        \renewcommand\arraystretch{1.2}

        \caption{ Results of QA accuracy of combining HittER and BERT in two Freebase-based question answering datasets. 
        % We report average scores and standard deviation from five random runs.
        }
        
        \scalebox{0.85}{
        
        \begin{tabular}{lcccc}
        
        \toprule
        
        \multirow{2}{*}{Dataset} & \multicolumn{2}{l}{\textbf{FreebaseQA}} & \multicolumn{2}{l}{\textbf{WebQuestionSP}} \\ \cline{2-5} 
         & Full & Filtered & Full & Filter \\
         
        \midrule
        
        BERT & 19.8 & 30.8 & 23.2 & 46.5 \\
        +HittER & 21.2 & \textbf{37.1} & 27.1 & 51.0  \\   
        
        \midrule
        
        +Relphormer & \textbf{28.0} & \textbf{37.1}  & \textbf{30.0} & \textbf{52.4}  \\
        
        \bottomrule

        \end{tabular}
        
        }
        
        \label{tab:kbqa}

\end{table}

        %   Seed    FBQA-full FBQA-filter   WebQA-full  WebQA-filter
        %   1       0.279
        %   3       0.277
        %   5       0.282
        %   7       0.274
        %   9       0.280

        

==> tables/KGRC.tex <==
\begin{table}[!t]
    \caption{Results of Recommendation on MovieLens.}
    \centering
    \scalebox{0.85}{
    % \resizebox{0.3\textwidth}{!}{
        \begin{tabular}{ccc}
            \toprule
            \textbf{Model}  & \textbf{Hits@1} & \textbf{MRR} \\
            \midrule
            % FPMC & 0.1079 & 0.2273 \\
            % GRU4Rec & 0.2021 & 0.3476 \\
            % Caser & 0.1232 & 0.2529 \\
            % SASRec & 0.2544 & 0.4026 \\
            % BERT4REC & 0.3440 & 0.4785  \\
            
            % FPMC & 0.11 & 0.23 \\
            % GRU4Rec & 0.20 & 0.35 \\
            % Caser & 0.12 & 0.25 \\
            % SASRec & 0.25 & 0.40 \\
            BERT4REC & 0.34 & 0.48  \\
            % + StAR &  &   \\
            % \midrule
            + \bizhen{KGBERT} & \textbf{0.36} & \textbf{0.49} \\
            \midrule
            + \bizhen{Relphormer} & \textbf{0.36} & \textbf{0.49}
            \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:rec}
    
\end{table} 

% \begin{table}[t]
% 	\centering
% 	\caption{\bizhen{ Performance comparison of all methods on MIND. 
%     The superscript $\ast$ indicates the improvement is statistically significant where $p$-value $<0.01$ level.}}
% 	\label{tab:results}
%     \scalebox{0.85}{
% 	\begin{tabular}{c|cc|cc}
 
%         \toprule
%         \multirow{2}{*}{Model} &\multicolumn{2}{c}{MIND} &\multicolumn{2}{c}{Amazon-book} \\
% 		~ &  Recall & NDCG &  Recall & NDCG \\
% 		\midrule
% 		BPR & 9.38\%$^\ast$ & 0.0469$^\ast$ \\ 
% 		NCF & 8.93\%$^\ast$ & 0.0436$^\ast$ \\ 
% 		GC-MC & 9.84\%$^\ast$ & 0.0491$^\ast$ \\
% 		LightGCN & 10.33\%$^\ast$ & 0.0520$^\ast$ \\
% 		SGL & 10.32\%$^\ast$ & 0.0539$^\ast$ \\
% 		CKE & 9.01\%$^\ast$ & 0.0382$^\ast$ \\
% 		RippleNet & 8.58\%$^\ast$ & 0.0407$^\ast$ \\
% 		KGCN & 8.87\%$^\ast$ & 0.0431$^\ast$ \\
% 		KGAT & 9.07\%$^\ast$ & 0.0442$^\ast$ \\
% 		KGIN & 10.44\%$^\ast$ & 0.0527$^\ast$ \\
% 		CKAN & 9.91\%$^\ast$ & 0.0499$^\ast$\\
% 		MVIN & 9.62\%$^\ast$ & 0.0487$^\ast$ \\
% 		KGCL & {10.73\%} & {0.0551} \\
%         \midrule
%         Relphormer & & \\
% 		\bottomrule
% 	\end{tabular}
% 	}
% 	% \vspace{-0.1in}
% \end{table}

% 实验部分 t2 t3
% 换页 两个qa 一个推荐 三个柱状图置顶;

% 同一页, 跟着case图;

% 换页：模型分析，attention图分析;


==> tables/LinkPrediction-Imbalance.tex <==
\begin{table}[]
        
        \caption{Results of imbalanced link prediction}
        
        \begin{tabular}{llllll}
            \toprule
        \multirow{3}{*}{\textbf{Model}} & \multicolumn{5}{c}{\multirow{2}{*}{Codex-large-imb}} \\
            & \multicolumn{5}{c}{} \\
            & Hits@1 & Hits@3 & Hits@ & MR & MRR \\
            \midrule
        TransE & & & & & \\
        RotatE  & & & & & \\
        KG-BERT & & & & & \\
        StaR & & & & & \\
        TeKo & & & & & \\
            \midrule
        Relphormer & & & & & \\
            \toprule
        \end{tabular}

\end{table}

==> tables/Model_Comparison.tex <==
\begin{table}[!t]
    % \begin{center}
%   \vspace{0.05cm}
 \caption{The difference between Relphormer and previous Transformer-based approaches for KGs.}
    % \small
    % \centering

    % \resizebox{0.5\columnwidth}{!}{
    \resizebox{0.45\textwidth}{!}{
    
    \begin{tabular}{lccc}
    \toprule
    Model & Graph Type & Graph Context & Task \\
    \midrule
    TransE & KG & No & Link Prediction \\
    Hitter & KG & Yes & Link Prediction \\
    KG-BERT & KG & No & Link Prediction \\
    Graphormer & Graph & Yes & Graph Classification \\
   Gophormer & Graph & Yes & Node Classification \\
    \midrule
    Relphormer (Ours)& KG & Yes & Link Prediction, QA, Rec. \\
    \bottomrule
    \end{tabular}
    
    }

    \label{tab:diff}
\end{table}

==> tables/ProteinPrediction.tex <==
\begin{table}[!t]
        \caption{Protein Function Prediction Results.}
        \centering
        \resizebox{0.4\textwidth}{!}{
            \begin{tabular}{ccc}
                \toprule
                \textbf{Model}  & \textbf{ROC-AUC} & \textbf{Params} \\
                \midrule
                GCN & 72.51 ± 0.35 & 96.9k \\
                GraphSAGE & 77.68 ± 0.2 & 193k \\
                DeeperGCN & 86.16 ± 0.16 & 2.37M \\
                UniMP & 86.42 ± 0.08 & 1.91M \\
                GAT & 86.82 ± 0.21 & 2.48M \\
                UniMP+CEF & 86.91 ± 0.18 & 1.96M \\
                RevGNN-Deep & 87.74 ± 0.13 & 20.03M \\
                RevGNN-Wide & 88.24 ± 0.15 & 68.47M \\
                ADGN & 88.65 ± 0.13 & 8.61M \\
                \midrule
                ADGN (TransE) &  & 8.61M \\
                ADGN (TransE) &  &  \\
                \midrule
                ADGN (Relphormer) &  & 8.61M \\
                ADGN (Relphormer) &  &  \\
                \bottomrule
            \end{tabular}
        }
    \end{table} 
